Evolving Transferable Neural Pruning Functions

Structural design of neural networks is crucial for the success of deep learning. While most prior works in evolutionary learning aim at directly searching the structure of a network, few attempts have been made on another promising track, channel pruning, which recently has made major headway in designing efficient deep learning models. In fact, prior pruning methods adopt human-made pruning functions to score a channel's importance for channel pruning, which requires domain knowledge and could be sub-optimal. To this end, we pioneer the use of genetic programming (GP) to discover strong pruning metrics automatically. Specifically, we craft a novel design space to express high-quality and transferable pruning functions, which ensures an end-to-end evolution process where no manual modification is needed on the evolved functions for their transferability after evolution. Unlike prior methods, our approach can provide both compact pruned networks for efficient inference and novel closed-form pruning metrics which are mathematically explainable and thus generalizable to different pruning tasks. While the evolution is conducted on small datasets, our functions shows promising results when applied to more challenging datasets, different from those used in the evolution process. For example, on ILSVRC-2012, an evolved function achieves state-of-the-art pruning results.

==> Supplementary_Material/func_validity.tex <==
\section{Function Validity}\label{sec:func_val}

The function expressions generated from mutation and crossover can be invalid (non-invertible matrix, dimension inconsistency, etc.) due to the random selections of operators, operands, and nodes in the expression trees. 
To combat this issue and enlarge our valid function space, 
some operators are deliberately modified from their standard definition. 
For instance, whenever we need to invert a positive semi-definite scatter matrix $S$, we automatically add a ridge factor $\rho I$, and invert the matrix $S + \rho I$. 
For dimension inconsistency in elementwise operations, we have two options to pad the operand with a smaller dimension: 
(1) with 0 for $+$ and $-$, and 1 for $\times$, and $\div$,
(2) with its own value if it is a scalar.
Moreover, 
we conduct a validity test on the mutated/crossovered functions every time after the mutation/crossover process.
The invalid expressions are discarded, and the mutation/crossover operations are repeated until we recover the population size with all valid functions.
These methods ensure we generate valid function expressions under our vast design space during the evolution process.


